DRGraph: An Efficient Graph Layout Algorithm for Large-scale Graphs by Dimensionality Reduction

Efficient layout of large-scale graphs remains a challenging problem: the force-directed and dimensionality reduction-based methods suffer from high overhead for graph distance and gradient computation. In this paper, we present a new graph layout algorithm, called DRGraph, that enhances the nonlinear dimensionality reduction process with three schemes: approximating graph distances by means of a sparse distance matrix, estimating the gradient by using the negative sampling technique, and accelerating the optimization process through a multi-level layout scheme. DRGraph achieves a linear complexity for the computation and memory consumption, and scales up to large-scale graphs with millions of nodes. Experimental results and comparisons with state-of-the-art graph layout methods demonstrate that DRGraph can generate visually comparable layouts with a faster running time and a lower memory requirement.

==> content/framework.tex <==
\begin{table}[!t]
   \centering
     \caption{Mathematical Notations}
   %\topcaption{Mathematical Notations}% requires the topcapt package
   \begin{tabular}{p{0.35\columnwidth}p{0.55\columnwidth}} % Column formatting, @{} suppresses leading/trailing space
      \hline
      Symbol & Description\\
      \hline
      $G=(V,E,A)$ & A graph\\
      $V=\{v_1, v_2,..., v_N\}$ & The node set \\
      $E=\{e_1, e_2,..., e_M\}$ & The link set\\
      $A$ & The adjacent matrix\\
      $Y=\{y_1,y_2,...,y_N\}$ & The layout positions of nodes\\
      $GD(G)$ & Graph distance\\
      $LD(Y)$ & Layout distance\\
      $TS(\cdot)$ & Topological similarity\\
      $LP(\cdot)$ & Layout proximity\\
      $D(\cdot,\cdot)$ & Distance function\\
      \hline
   \end{tabular}
  %    \caption{Mathematical Notations}
   \label{tab:notations}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
%\begin{adjustwidth}{-.15in}{0in}  
\centering
\caption{Our graph layout scheme unifies previous graph layout algorithms as specific cases with different choice of similarity and distance function.}
\label{table:summary}
\begin{tabular}{|c|c|l|l|l|l|l|}
\hline
 &  & FR~\cite{fruchterman1991graph} & KK~\cite{kamada1989algorithm} & Linlog~\cite{noack2003energy} & LINE~\cite{tang2015line} & Ours \\ \hline
\multirow{2}{*}{\makecell{Topological\\Similarity}} & \makecell{Graph\\Distance} & $GD_{ij}=A_{ij}$ & Shortest path length & $GD_{ij}=A_{ij}$ & \makecell[l]{$GD^1_{ij}=EdgeWeight_{ij}$\\$GD^2_{ij}=\frac{GD^1_{ij}}{OutDegree_{i}}$} & Shortest path length \\ \cline{2-7} 
 & \makecell{Similarity\\Function} & $TS_{ij} = GD_{ij}LD_{ij}^3/3c$ & $TS_{ij}=GD_{ij}$ & $TS_{ij}=GD_{ij}$ & $TS_{ij}=GD_{ij}$ & Gaussian distribution \\ \hline
\multirow{2}{*}{\makecell{Layout\\Proximity}} & \makecell{Layout\\Distance} & $LD_{ij}=\|y_i-y_j\|_2$ & $LD_{ij}=\|y_i-y_j\|_2$ & $LD_{ij}=\|y_i-y_j\|_2$ & $LD_{ij}=y_i^Ty_j$ & $LD_{ij}=\|y_i-y_j\|_2$ \\ \cline{2-7} 
 & \makecell{Proximity\\Function} & $LP_{ij} = c^2\log LD_{ij}$ & $LP_{ij}=LD_{ij}$ & $LP_{ij}=1/LD_{ij}$ & \makecell[l]{$LP^1_{ij}=sigmoid$\\$LP^2_{ij}=softmax$} & t-Student distribution \\ \hline
\makecell{Distance\\Mnimization} & \makecell{Distance\\Function} & $\sum_{ij}(TS_{ij}-LP_{ij})$ & $\sum_{ij}\frac{(TS_{ij}-LP_{ij})^2}{TS_{ij}^2}$ & $Dis_{IS}(TS||LP)$ & \makecell[l]{$Dis_{KL}(TS^1||LP^1)+$\\$Dis_{KL}(TS^2||LP^2)$} & $Dis_{KL}(TS||LP)$ \\ \hline
\end{tabular}
%\end{adjustwidth}
\end{table*}
%%1/(1+e^{-gd_{ij}}) 

\section{DRGraph}
%Previous works have discussed the equivalence between spring-electrical, energy based graph layout methods~\cite{noack2003energy} and equivalence between energy and dimensionality reduction based algorithms~\cite{yang2014optimization}.
Let $G = (V, E, A)$ be an undirected graph with a set of nodes $V=\{v_1, v_2,..., v_N\}$, a set of links $E=\{e_1, e_2,..., e_M\}$ and an adjacent matrix $A$. 
Each link is a connection between two nodes $e_m=(v_i,v_j) \in V \times V $. 
The adjacent matrix encodes link weight between nodes: $A_{ij}=1$ if $(v_i,v_j) \in E$.
Then, graph layout problem is simplified as embedding a given graph to two-dimensional space: $\phi: G \to Y, Y=\{y_1,y_2,...,y_N\}$, $y_n \in R^2$, where $y_n$ is the 2D position of node $v_n$.
Table \ref{tab:notations} lists the notations used in this paper.
%The main concept of graph layout is preserving the neighborhood in layout result.

In this section, we present a graph layout scheme which unifies force directed algorithms and dimensionality reduction based graph layout methods.
The existing graph layout algorithms (e.g., FR~\cite{fruchterman1991graph}, KK~\cite{kamada1989algorithm} and tsNET~\cite{kruiger2017graph}) are subsumed as special cases within our scheme.
These methods are tied by an optimization problem which minimizes the difference of property between the graph space and the layout space.
Topological similarity is defined as the pairwise similarity between two nodes in the graph space and layout proximity is defined as the pairwise proximity between two nodes in the layout space.
Connected nodes with larger topological similarity should be closer to each other in the layout space.
We employ a loss function to minimize the difference between topological similarity in the graph space and layout proximity in the layout space, in which the topological similarity is preserved as much as possible.
Generally, the scheme decomposes graph layout algorithm into three stages:
\begin{itemize}
    \item \textbf{Topological Similarity $TS$}: compute topological similarity probability between nodes by graph-theoretic distance in the graph space;
    \item \textbf{Layout Proximity $LP$}: measure layout proximity probability between nodes' positions based on the layout result;
    \item \textbf{Distance Minimization $Dis(TS,LP)$}: minimize the distance between topological similarity and layout proximity.
\end{itemize}



\subsection{Topological Similarity}
To visualize graph data, the graph structures must be maintained in graph layout space.
We define the topological similarity to encodes the graph distance $GD(G) \in R^{V\times V} $ between nodes.
Nodes with small graph distance encodes their strong connection in the graph space.
In other words, we need to preserve the connection (graph distance) between nodes and their neighbors in graph layout.
%The graph distance includes graph-theoretic distance such as shortest path length and degree centrality.
There are three variations of graph distance defined in the graph space:
\begin{itemize}
    \item Shortest Path Length: Shortest path is widely employed in previous graph layout methods. Shortest path length usually implies the distance of two nodes in a real-world network.
    \item Link Connection: Only nodes that are neighbours should be drawn near each other. All the distances between connected nodes are set as 1.
    \item Embedding distance: Graph embedding methods~\cite{cai2017comprehensive} are adopted to project nodes into high-dimensional space, we usually use Euclidean distance or cosine distance to describe the graph distance.
\end{itemize}

Then, we transform graph distance to topological similarity by $TS(\cdot) \in R^{V\times V}$, where $TG(\cdot)$ is the similarity function.
We denote $TS_{ij}$ as the similarity between $i$-th node and $j$-th node.
We can design different similarity functions to capture useful features and remove noise of graph distance.
For instance, Gaussian distribution could be adopted to transform small graph distance into high similarity.
For spring-electrical based approaches, similarity encodes the attractive energy which is defined as the integration of attractive forces along the link: $TS_{ij} = \int f^a(x)dx$.
For energy-based approaches, we usually use graph distance directly: $TS_{ij} = GD_{ij}$.
Graph distances are also transformed into the probability of picking a link using non-linear dimensionality reduction methods (e.g. the normalized Gaussian distribution in tsNET \cite{kruiger2017graph}).

\subsection{Layout Proximity}
The second stage is the definition of layout proximity between nodes on layout space. 
The layout distance is defined as the distance between nodes in layout space.
We measure pairwise layout distance $LD(Y) \in R^{V\times V}$ between nodes' positions.
The choice of layout distance function is limited to human perception.
Therefore, we usually set layout distance as the Euclidean distance for visualization: $LD_{ij}(Y) = \|y_i-y_j\|_2$.
Graph embedding methods (e.g, Deepwalk~\cite{perozzi2014deepwalk}, node2vec~\cite{grover2016node2vec}, LINE~\cite{tang2015line}) usually measure the distance between two nodes by cosine distance.

Layout proximity is defined as the "closeness" between nodes based layout result.
We measure layout proximity probabilities as $LP(LD)\in R^{V\times V}$, where $LP(\cdot)$ is proximity function.
Likewise, proximity function captures important locality properties in layout space, providing an appropriate scale to connect topological similarity $TS$ and layout proximity $LP$.
For spring-electrical based approaches, proximity is defined as the integration of repulsive forces along the link: $TS_{ij} = \int f^r(x)dx$. 
We usually utilize graph distance directly in energy-based approaches. 
For graph layout by non-linear dimensionality reduction methods, we transform the layout distance to the probability by Gaussian distribution or t-Student distribution.

\subsection{Distance Minimization}
In this stage, our scheme is intended to minimize the distance between topological similarity and layout proximity.
For instance, Two nodes with high topological similarity should have a high layout proximity in layout space.
We adopt a distance function the measure the difference between two matrixes such as the stress function, Kullback-Leibler (KL) divergence and Itakura-Saito (IS) divergence.
\begin{eqnarray*}
D_{stress}(TS||LP) &=& \sum_{i,j}TS_{ij}^\alpha (TS_{ij}-LD_{ij})^2\\
D_{KL}(TS||LP) &=& \sum_{i,j}TS_{ij}\log \frac{TS_{ij}}{LD_{ij}}\\
D_{IS}(TS||LP) &=& \sum_{i,j}(\frac{TS_{ij}}{LD_{ij}} - ln \frac{TS_{ij}}{LD_{ij}} -1)
\end{eqnarray*}
We model the difference as an object function $O(TS||LP)$ and formulate graph layout problem as optimizing the loss function by searching a state with minimum loss:
\begin{eqnarray*}
Y^* &=& \argmax O(TS||LD)\\
&=&\argmax_{Y}  Dis(TS(GS(G),LP(LD(Y)))
\end{eqnarray*}

% \subsection{Special cases}
% Different selection of graph distance $GD(\cdot)$, layout distance $LD(\cdot)$, similarity function $TS(\cdot)$, proximity $LS(\cdot)$ and $Dis$ give different graph layout methods. Table \ref{table:summary} shows the summary of function selection of prioritized methods that have been widely used.

% For spring-electrical based approaches such as FR by Fruchterman and Reingold \cite{fruchterman1991graph}, topological similarity is potential energy of attraction and layout proximity is potential energy of repulsion. The energy is defined as the integration of force along the link. Similarity function is defined as $TS(GD_{ij}) = GD_{ij}^3/3c$, where $GD_{ij} = A_{ij}$. Proximity function is set as $LP(GD_{ij}) = c^2*\log(GD_{ij})$ with layout distance $GD_{ij} = \|y_i-y_j\|_2$. The loss function is defined as the sum of difference between attractive energy and repulsive energy: $O(TS||LP)= \sum_{ij}(TS_{ij}-LP_{ij})$. The gradient of the object funtion is the sum of attractive and repulsive forces: $\frac{\partial O}{d_{ij}}= \sum_{j}(A_{ij}GD_{ij}^2/c - c^2/LD_{ij})=\sum (f^a - f^r)$.

% Energy based methods such as KK by Kamada and Kawai \cite{kamada1989algorithm}, object function is defined as the residual sum of squares between shortest path length and Eucilidean distance: $O(TS||LP)= TS_{ij}^{-2}(TS_{ij}-LP_{ij})^2 = GD_{ij}^{-2}(GD_{ij}-LD_{ij})^2$.

% Linlog method computes topological similarity as $TS_{ij}=GD_{ij}=A_{ij}$ and layout proximity as $LP_{ij}=1/LD_{ij}$ where $LD_{ij} = \|y_i-y_j\|_2$. We adopt IS divergence to model the object function: $O(TS||LP) = D_{IS}(TS||LP) = \sum_{i,j}(\frac{TS_{ij}}{LP_{ij}} - ln \frac{TS_{ij}}{LP_{ij}} -1) = \sum_{ij}(LD_{ij}-ln~LD_{ij} -1)$.

% Graph layout method tsNET adopts Gaussian distribution to transform the shortest path length into the topological similarity probability.
% %: $$p_{ij}(gd_{ij}) = exp(-gd_{ij}^2/2\sigma^2)/\sum_{kl}exp(-gd_{kl}^2/2\sigma^2)$$ 
% Likewise, layout proximity is measured by t-Student distribution.
% %$$q_{ij}(ld_{ij}) = (1+ld_{ij}^2)^{-1}/\sum_{kl}(1+ld_{kl}^2)^{-1}$$
% The loss function is defined on KL distance:
% $O(TS||LP)=\lambda_{KL}D_{KL}(TS||LP)+\frac{\lambda_c}{2N}\sum_i\|y_i\|^2-\frac{\lambda_r}{2N^2}\sum_{i,j}log(\|y_i-y_j\|^2)$.
% % \begin{eqnarray*}
% % \frac{\partial O}{y_i} &=& 4(-\sum_{j \neq i}fa_{ij}+\sum_{j \neq i}fr_{ij})\\
% % fa_{ij} &=& \frac{p_{ij}ld_{ij}}{1+ld_{ij}^2}\\
% % fr_{ij} &=& \frac{q_{ij}ld_{ij}}{1+ld_{ij}^2}\\ 
% % \end{eqnarray*}
% %where $fa_{ij}$ denotes the attractive force between $y_i$ and $y_j$ and $fr_{ij}$ represents the repulsive force. In this way, graph layout method by t-SNE is another version of spring-electrical model.












==> content/method320.tex <==
\section{DRGraph}
%In this section, we present an efficient graph layout algorithm DRGraph.
%We first provide an overview of our algorithm.
%Then, we introduce how to approximate sparse node similarity with a sparse distance matrix, estimate the gradient using mini-batch strategy and accelerate the optimization process by leveraging multi-level approach.
%We discuss the computational complexity of DRGraph and show the advantages over conventional methods.

\begin{table}[!t]
   \centering
     \caption{Mathematical Notations}
   \begin{tabular}{p{0.35\columnwidth}p{0.55\columnwidth}} % Column formatting, @{} suppresses leading/trailing space
      \hline
      Symbol & Description\\
      \hline
      $G=(V,E,A)$ & A graph\\
      $V=\{v_1, v_2,..., v_N\}$ & The node set \\
      $E=\{e_1, e_2,..., e_M\}$ & The link set\\
      $A$ & The adjacent matrix\\
      $Y=\{y_1,y_2,...,y_N\}$ & The layout positions of nodes\\
      $GD(G)$ & Graph distance\\
      $LD(Y)$ & Layout distance\\
      $NS(\cdot)$ & Node similarity\\
      $LP(\cdot)$ & Layout proximity\\
      $D(\cdot,\cdot)$ & Distance function\\
      $NNG(v_i,k)$ & $k$-order nearest neighbor in graph space\\
      $NNL(y_i,k)$ & $k$-nearest neighbor in layout space\\
      \hline
   \end{tabular}
   \label{tab:notations}
\end{table}

\subsection{Overview}
Formally, let $G = (V, E, A)$ be an undirected unweighted graph with a set of nodes $V=\{v_1, v_2,..., v_{|V|}$, a set of links $E=\{e_1, e_2,..., e_{|E|}\}$ and an adjacent matrix $A$. 
Each link is a connection between two nodes $e=(v_i,v_j) \in V \times V $. 
The adjacent matrix encodes link between nodes: $A_{ij}=1$ if $(v_i,v_j) \in E$.
Then, graph layout problem is formulated as embedding a given graph to two-dimensional space: $\phi: G \to Y, Y=\{y_1,y_2,...,y_{|V|}\}$, $y_n \in R^2$, where $y_n$ is the position of node $v_n$.
Table \ref{tab:notations} lists the notations used in this paper.

Graph layout is tied by an optimization problem~\cite{yang2014optimization} which minimizes the property difference between the graph space and the layout space.
Node similarity $NS$ is defined as the pairwise similarity between two nodes in the graph space and layout proximity $LP$ is defined as the pairwise proximity between two nodes in the layout space.
Connected nodes with large node similarity should have large layout proximity in the layout space.
A loss function $D(NS,LP)$ is employed to model the difference between node similarity and layout proximity, in which the node similarity is preserved as much as possible.
Generally, our graph layout algorithm consists of three stages:
\begin{itemize}
    \item \textbf{Node Similarity $NS(GD)$}: compute node similarity probability between nodes by graph-theoretic distance $GD$ in the graph space;
    \item \textbf{Layout Proximity $LP(LD)$}: measure layout proximity probability using the layout distance $LD$ between nodes' positions in the layout space;
    \item \textbf{Difference Minimization $min~D(NS,LP)$}: minimize the difference between node similarity and layout proximity.
\end{itemize}
%DRGraph is capable of capturing local neighborhoods due to the selection of similarity and proximity functions.

\subsection{Node Similarity}
To visualize graph data, the graph structures must be maintained in the layout space.
Shortest path length usually implies the distance of two nodes in a real-world network.
Nodes with small graph distance encodes their strong connection in the graph space.
We compute graph distance $GD$ as shortest path length by breadth-first-search (BFS): $GD_{ij} = BFS(G,v_i,v_j), GD(G) \in R^{V\times V}$.

Then, we transform graph distance to node similarity by $NS(GD) \in R^{V\times V}$, where $NS(\cdot)$ is the similarity function.
We denote $NS_{ij}$ as the similarity between $i$-th node and $j$-th node.
To preserve locality properties, we convert graph distance in graph space into probabilities that represent node similarity.
The node similarity between two nodes is given by Gaussian distribution:
\begin{eqnarray*}
NS_{j|i}&=&\frac{exp(-GD_{ij}^2/2\sigma_i^2)}{\sum_{k\not=i}exp(-GD_{ik}^2/2\sigma_i^2)}\\
NS_{i|i}&=&0\\
NS_{ij}&=&\frac{NS_{j|i}+NS_{j|i}}{2|V|}
\end{eqnarray*}
where $GD_{ij}$ is shortest path length between vertices $v_i$ and $v_j$ and $\sigma_i$ is the variance of Gaussian distribution on data $v_i$.
%The value of $\sigma_i$ is computed by binary search or specified by users.
% to describe the distribution of node similarity over each node $v_i$.


\textbf{Node Similarity Approximation}
However, all pairwise shortest path length between $|V|$ nodes requires $O(|V|(|V|+|E|))$ computation using breadth-first-search. 
In addition, Node similarity computation requires $O(|V|^2)$ computation, because their normalization terms sum over all $|V|^2$ pairs of nodes.

We can approximate node similarity using a sparse representation without a significant effect on the quality of graph layout.
Because, for two nearby nodes with small shortest path length, its node similarity is relatively high according the definition.
In contrast, the node similarity between widely separated nodes will be almost infinitesimal.
Small shortest path length has much larger importance in DRGraph.
%For two nodes with large shortest path length, their node similarity computed by Gaussian kernel are nearly infinitesimal. 
Therefore, we just compute the node similarity between each node and its neighbors instead of all other nodes.

We define $k$-order nearest neighbors $NNG(v_i,k)$ of node $v_i$ as a set of nodes whose shortest path length is less than or equal to $k$:
$$NNG(v_i,k) = \{v| BFS(G,v_i,v) \leq k, v \in V\} $$
For instance, $1$-order nearest neighbors $NNG(v_i,1)$ is the set of nodes connected to node $v_i$.
The node similarity $NS_{ij}$ is reformulated as: 
\begin{eqnarray*}
NS_{j|i}&=&\left\{
\begin{aligned}
\frac{exp(-GD_{ij}^2/2\sigma_i^2)}{\sum_{k\not=i}exp(-GD_{ik}^2/2\sigma_i^2)}&,&~if~v_j \in NNG(v_i,k)\\
0&,& ~otherwise\\
\end{aligned}
\right.\\
NS_{ij}&=&\frac{NS_{j|i}+NS_{j|i}}{2|V|}
\end{eqnarray*}                                                             

%We define the edge connection as the first order neighbors: $$N_1(v)=\{u|(u,v)\in E\}$$
%For each pair of nodes linked by an edge $(u,v)$, the shortest path length between $u$ and $v$ is set as 1. The $k$-th order neighbors are defined as a set of nodes who have a edge connection with $k-1$-th order neighbors: $$N_k(v) = \{u|(u,w)\in E, w\in N_{k-1}(v), u\not\in \cup_{i=1}^{k-1}N_{i}(v)\}$$ The shortest path length between $u$ and $v \in N_k(v)$ is set as $k$.
%We define K-nearest neighbor set of each node as a set of nodes that have shortest path length: 
%$KNN(v) = \cup_{i=1}^{k}N_{i}(v_i), \cup_{i=1}^{k}|N_{k}|<K<\cup_{i=1}^{k}|N_{k+1}|$
\subsection{Layout Proximity}
Layout proximity is defined as the "closeness" between nodes in layout result space.
We first compute layout distance $LD$ as Euclidean distance between nodes' positions:
$LD(Y) \in R^{V\times V},~LD_{ij}=\|y_i-y_j\|_2$.


Then, we measure layout proximity as $LP(LD)\in R^{V\times V}$, where $LP(\cdot)$ is proximity function.
Proximity function captures important locality properties in layout space, providing an appropriate scale to connect node similarity $NS$ and layout proximity $LP$.
For layout proximity, we measure the probability of the pair $(y_i,y_j)$ in the layout space with Student's t-distribution.
The Student's t-distribution is employed by t-SNE to capture local proximity within groups.
Therefore, layout proximity can be formulated as follows: 
$$LP_{ij}=\frac{(1+LD_{ij}^2)^{-1}}{\sum_{k\not=l}(1+LD_{ij}^2)^{-1}}$$
%= \frac{(1+ld_{ij}^2)^{-1}}{Z}$$
%where $Z$ denotes the normalization term.





% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
%\begin{adjustwidth}{-.15in}{0in}  
\centering
\caption{Comparison between DRGraph and conventional graph layout methods based on different choice of similarity and distance function. $D_{IS}$ denotes Itakura-Saito divergence.}
\label{table:summary}
\begin{tabular}{|c|c|l|l|l|l|l|}
\hline
 &  & FR~\cite{fruchterman1991graph} & KK~\cite{kamada1989algorithm} & Linlog~\cite{noack2003energy} & tsNET~\cite{kruiger2017graph} & Ours \\ \hline
 
\multirow{2}{*}{\makecell{Node\\Similarity}} &
\makecell{Graph\\Distance} &
$GD_{ij}=A_{ij}$ &
Shortest path length &
$GD_{ij}=A_{ij}$ &
\makecell[l]{All pairwise\\shortest path length}&
\makecell[l]{Shortest path length\\between neighbors} \\ \cline{2-7} 

 & \makecell{Similarity\\Function} & $NS_{ij} = GD_{ij}LD_{ij}^3/3c$ & $NS_{ij}=GD_{ij}$ & $NS_{ij}=GD_{ij}$ & Gaussian distribution & Gaussian distribution \\ \hline
 
\multirow{2}{*}{\makecell{Layout\\Proximity}} & \makecell{Layout\\Distance} & $LD_{ij}=\|y_i-y_j\|_2$ & $LD_{ij}=\|y_i-y_j\|_2$ & $LD_{ij}=\|y_i-y_j\|_2$ & \makecell[l]{All pairwise\\Euclidean distance} & \makecell[l]{Euclidean distance\\ between sampled nodes} \\ \cline{2-7} 

 & \makecell{Proximity\\Function} & $LP_{ij} = c^2\log LD_{ij}$ & $LP_{ij}=LD_{ij}$ & $LP_{ij}=1/LD_{ij}$ & t-Student distribution & t-Student distribution \\ \hline
 
\makecell{Difference\\Mnimization} & \makecell{Distance\\Function} & $\sum_{ij}(NS_{ij}-LP_{ij})$ & $\sum_{ij}\frac{(NS_{ij}-LP_{ij})^2}{NS_{ij}^2}$ & $D_{IS}(NS||LP)$ & $D_{KL}(NS||LP)$ & $D_{KL}(NS||LP)$ \\ \hline

\end{tabular}
%\end{adjustwidth}
\end{table*}




\subsection{Difference Minimization}
In this stage, our algorithm is intended to minimize the difference between node similarity and layout proximity.
For instance, Two nodes with high node similarity should have a high layout proximity in layout space.
In others words, nodes with short graph distance should be close to each other in the layout space.
The Kullback-Leibler divergence function is adopted to measure the difference between node similarity and layout proximity.
We model the difference as an object function $O(NS||LP)$ and formulate graph layout problem as optimizing the object function by searching a state with minimum loss:
\begin{eqnarray*}
Y^* &=& \argmin O(NS||LP)\\
&=&\argmin_{Y}  D_{KL}(NS(GD(G),LP(LD(Y)))\\
&=& \argmin_Y \sum_{i,j}NS_{ij}\log \frac{NS_{ij}}{LP_{ij}}\\
&=& \argmin_Y \sum_{i\not=j} NS_{ij}\log NS_{ij} - NS_{ij}\log LP_{ij}
\end{eqnarray*}
Since the first term is a constant, the problem is equivalent to the following optimization problem:
$$Y^* = \argmax_Y \sum_{i\not=j} \quad NS_{ij}\log LP_{ij}$$
%such as the stress function, Kullback-Leibler (KL) divergence and Itakura-Saito (IS) divergence.
%\begin{eqnarray*}
%D_{stress}(NS||LP) &=& \sum_{i,j}NS_{ij}^\alpha (NS_{ij}-LD_{ij})^2\\
%D_{KL}(NS||LP) &=& \sum_{i,j}NS_{ij}\log \frac{NS_{ij}}{LD_{ij}}\\
%D_{IS}(NS||LP) &=& \sum_{i,j}(\frac{NS_{ij}}{LD_{ij}} - ln \frac{NS_{ij}}{LD_{ij}} -1)
%\end{eqnarray*}
%In the third stage, similar vertices should be close to each other in the layout space, the optimal choice of layout is to minimize Kullback-Leibler divergences between node similarity $P$ and layout proximity $Q$. The problem boils down to solving the following problem:
% \begin{eqnarray*}
% Y^* &=& \argmin_Y O(P||Q)\\
% &=& \argmin_Y Dis_{KL}(P||Q)\\
% &=& \argmin_Y \sum_{i\not=j} p_{ij}\log \frac{p_{ij}}{q_{ij}}\\
% &=& \argmin_Y \sum_{i\not=j} p_{ij}\log p_{ij} - p_{ij}\log q_{ij}
% \end{eqnarray*}
\textbf{Gradient Estimation}
In previous method such as tsNET, we need to compute $|V|^2$ Euclidean distances to construct layout proximity.
To reduce the number of Euclidean distance computations, we employ negative sampling technique to estimate the gradient using a small set of sampled nodes.
Negative sampling technique samples 1 positive node and $M$ negative nodes for each node.
A logistic regression is employed to separate positive $y_j$ and negative nodes $y_{j_m}$:
$$\log LP_{ij} + \sum^{M}_{m=1}\gamma \log (1-LP_{ij_m})$$
We can compute the gradient of each node with $1+M$ Euclidean distances.
Negative sampling technique reduce distance calculation from $O(N)$ to $O(M)$ for the gradient computation of each node.
Therefore, the optimization problem is reformulated as follows:
\begin{eqnarray}\label{eq:objectfunction}
Y^*   &=& \argmax_Y \sum_{i\not=j} NS_{ij}[\log LP_{ij}+\sum\limits_{k=1}^M \gamma \log(1-LP_{ij_m})]
\end{eqnarray}
The partial derivative of equation (\ref{eq:objectfunction}) by $y_j$ is derived as:
\begin{eqnarray*}
\frac{\partial O}{\partial y_i} &=& -F^{attr}_{ij} + \sum\limits_{m=1}^M \gamma F^{rep}_{ij_m}\\
F^{attr}_{ij} &=& \frac{2NS_{ij}(y_i-y_j)}{1+LD_{ij}^2}=\frac{2NS_{ij}(y_i-y_j)}{1+(y_i-y_j)^2}\\
F^{rep}_{ij_m} &=& \frac{2\gamma NS_{ij}(y_i-y_{j_m})}{LD_{ij_m}^2(1+LD_{ij_m}^2)} = \frac{2\gamma NS_{ij}(y_i-y_{j_m})}{(y_i-y_{j_m})^2(1+(y_i-y_{j_m})^2)}
\end{eqnarray*}
The gradient shows that each node receives $1$ attractive force and $M$ repulsive forces.
%To solve optimization problem, we randomly select two vertices and samples M negative points ($y_{j_k}$) by adopting negative sampling technique used in LargeVis.

\subsection{Multilevel Optimization}
The multilevel approach has been used widely in many graph layout methods~\cite{gajer2000grip,hachul2004drawing}. 
With the multilevel approach, we can find a global optimal layout of a coarse graph, provide a better initial layout for finer graph and optimize the object function with less iteration.
The multilevel approach consists of three steps~\cite{hu2005efficient}: coarsening, coarsest graph layout and refinement.


\textbf{Graph Coarsening}
In the coarsening step, a series of coarse graph $G^0, G^1 ,G^2,...,G^L$ with decreasing sizes are generated, where $G^0$ is the original graph and $G^L$ is the coarsest graph.
Given a graph $G_l=(V^l,E^l)$, we partition the node set of G into disjoint subsets.
First, we randomly select a node $v^l_i$. 
Then $v^l_i$ and its $1$-order neighbors are coalesced into one new node in $G_{l+1}$.
This process is repeated until all nodes have been assigned to new nodes.
At last, we keep edge $(v^l_i,v^l_j)$ in the new graph, if $v^l_i$ and $v^l_j$ are coalesced into two different nodes in $G_{l+1}$.

\textbf{Coarsest Graph Layout}
For the coarsest graph $G^L$, we layout the graph using DRGraph with a random initial.
The optimal layout of the coarsest graph can be found cheaply.

\textbf{Refinement}
Once the graph layout of a coarse graph $G^l$ is generated, the initial layout of the finer graph $G^{l-1}$ is derived from $G^l$.
The position of a node in $G^{l-1}$ is set as the position of its parent node in $G^l$.
Then, we recursively refine the layout of a finer graph using DRGraph until the original graph $G^0$ has been refined.
%In the refinement step, we recursively refine a finer graph $G^l$ with an initial layout from graph $G^{l+1}$. 


\subsection{Complexity Analysis}
\textbf{Time Complexity}
The time complexity of our algorithm includes $k$-order nearest neighbor set searching, node similarity computation and optimization.
The $k$-order nearest neighbor set are found in $O(C|V|),~C=min(|V|,degree_{avg}^k),~degree_{avg}=|E|/|V|$, where $degree_{avg}$ denotes the average degree.
In addition, it is infeasible to measure and store node similarity with too large nearest neighbor set for graphs with millions nodes due to the memory limitation.
In most instances, $1$-order nearest neighbors are sufficient to capture neighborhood information and generate pleasing graph layout results.
We can find $1$-order nearest neighbor set in $O(E)$ time.

For node similarity computation, the value of graph distances $GD_{ij}$ between $v_i$ and $NNG(v_i,k)$ range from 1 to k for node $v_i$. 
We can pre-compute Gaussian distribution for k different values and measure $NS_{ij}$ with $2k$ calculations.
Therefore, our method uses the nearest neighbor set to compute node similarity in $O(k|V|)$ time.
The node similarity can be measured in $O(|V|)$ if we employ $1$-order nearest neighbors.

Each optimization iteration takes $O(M)$ time, where $M$ is the number of negative samples. 
In practice, we find that the number of iterations $T$ used for optimization is usually proportional to the number of nodes $|V|$.
For instance, a reasonable number of iterations for 1 million nodes is 5k million.
The time complexity of optimization is $(TM|V|)$.
Therefore, the total time complexity of the DRGraph is $O(C|V|+k|V|+TM|V|)$. 
We are able to reduce the time complexity to $O(|E|+|V|+TM|V|)$ if we employ $1$-order nearest neighbor set.

\textbf{Space Complexity}
DRGraph requires only $O(C|V|)$ memory to store spare node similarity and $O(|V|)$ memory to store the layout position of nodes.
We can reduce the space complexity of DRGraph to $O(|E|+|V|)$ if we employ $1$-order nearest neighbor set.

%DRGraph requires only $O(|E|)$ memory to store node similarity with $1$-order nearest neighbor set and $O(|V|)$ memory to store the layout position of nodes.
%Therefore, the total time complexity of the DRGraph is $O(|E|+k|V|+TM|V|)$ and space complexity is $O(|E|+|V|)$ if we employ $1$-order nearest neighbor set.

%Compared to force-directed methods, 

%Compared to tsNET, time complexity

\subsection{Comparisons}
Graph layout methods are tied by an optimization problem which minimizes the difference of property between the graph space and the layout space~\cite{yang2014optimization}.
The difference between graph layout methods is owing to the selection of similarity, proximity and distance functions.
Table \ref{table:summary} shows the summary of function selection of benchmark methods that have been widely used.

\textbf{Force-directed based}
For spring-electrical based approaches such as FR by Fruchterman and Reingold \cite{fruchterman1991graph}, node similarity is potential energy of attraction and layout proximity is potential energy of repulsion. 
The energy is defined as the integration of force along the link. 
The loss function is defined as the sum of difference between attractive energy and repulsive energy.
Therefore, the gradient of the object function is the sum of attractive and repulsive forces
The main weakness of spring-electrical model is that long edge with large energy takes much more importance in object function. 
As a result, they may easily converge to local minima and they are not good at preserving the local structure of data.  

The object function of energy based methods such as KK by Kamada and Kawai \cite{kamada1989algorithm} is defined as the residual sum of squares between shortest path length in graph space and Eucilidean distance in layout space.
The KK algorithm requires the computation of all pairwise shortest path length.
Thus, it is still far from satisfaction when applied to large-scale data.

\textbf{Dimensional reduction based}
We choose the same functions used in tsNET to keep the neighbor-preserving nature of t-SNE.
In contrast to tsNET, DRGraph utilizes spare similarity representation and negative sampling technique to accelerate the computation.
DRGraph achieves significantly performance over tsNET in both computational and memory complexity while producing a comparable solution quality.

==> content/method_old.tex <==
\section{Method}
In this section, we present DRGraph, an efficient graph layout algorithm based on our scheme.
DRGraph is capable of capturing local neighborhoods due to the selection of similarity and proximity functions.
As shown in Table \ref{table:summary}, we chooses graph distance as shortest path length, similarity function as Guassian distribution, layout distance as Euclidean distance, proximity function as t-Student distribution and distance function as KL divergence.
We uses nearest neighbors to approximate topological similarity by a sparse representation and approximates the gradients of object function using negative sampling technique.
At last, we discuss the computational complexity of our model and shows the advantage over previous methods.




Given an unweighted graph, our method follows three stages: topological similarity, layout proximity and distance minimization.

\subsection{Topological Similarity}
At first, we compute graph distance as shortest path length by Breadth-First-Search (BFS): $GD_{ij} = BFS{G}(v_i,v_j)$.
To preserve locality properties, we convert graph distance in graph layout space into probabilities that represent topological similarity.
For nearby nodes with small shortest path length, its topological similarity is relatively high.
In contrast, the topological similarity between widely separated nodes will be almost infinitesimal.
Therefore, small shortest path length has much larger importance in DRGraph.
The topological similarity between two nodes is given by Gaussian distribution:
\begin{eqnarray*}
TS_{j|i}&=&\frac{exp(-GD_{ij}^2/2\sigma_i^2)}{\sum_{k\not=i}exp(-GD_{ik}^2/2\sigma_i^2)}\\
TS_{i|i}&=&0\\
TS_{ij}&=&\frac{TS_{j|i}+TS_{j|i}}{2|V|}
\end{eqnarray*}
where $GD_{ij}$ is shortest path length between vertices $v_i$ and $v_j$ and $\sigma_i$ is the variance of Gaussian distribution on data $v_i$.
The value of $\sigma_i$ is computed by binary search or specified by users.% to describe the distribution of topological similarity over each node $v_i$.
\textbf{Acceleration}
However, all pairwise shortest path length between $|V|$ nodes requires $O(|V|(|V|+|E|))$ computation using Breadth-First-Search. Topological similarity computation requires $O(|V|^2)$ computation, because their normalization terms sum over all $|V|^2$ pairs of nodes.
For two nodes with large shortest path length, their topological similarity computed by Gaussian kernel are nearly infinitesimal. Therefore, we can approximate topological similarity using a sparse representation without a significant effect on the quality of graph layout.
We redefine the topological similarity between each node and its neighbors instead of all other nodes.

We define the edge connection as the first order neighbors: $$N_1(v)=\{u|(u,v)\in E\}$$
For each pair of nodes linked by an edge $(u,v)$, the shortest path length between $u$ and $v$ is set as 1. The $k$-th order neighbors are defined as a set of nodes who have a edge connection with $k-1$-th order neighbors: $$N_k(v) = \{u|(u,w)\in E, w\in N_{k-1}(v), u\not\in \cup_{i=1}^{k-1}N_{i}(v)\}$$ The shortest path length between $u$ and $v \in N_k(v)$ is set as $k$.
We define K-nearest neighbor set of each node as a set of nodes that have shortest path length: 
$KNN(v) = \cup_{i=1}^{k}N_{i}(v_i), \cup_{i=1}^{k}|N_{k}|<K<\cup_{i=1}^{k}|N_{k+1}|$
The topological similarity $p_{ij}$ is reformulated as: 
\begin{eqnarray*}
p_{j|i}&=&\left\{
\begin{aligned}
\frac{exp(-gd_{ij}^2/2\sigma_i^2)}{\sum_{k\not=i}exp(-gd_{ik}^2/2\sigma_i^2)}&,&~if~v_j \in N(v)\\
0&,& ~otherwise\\
\end{aligned}
\right.\\
p_{ij}&=&\frac{p_{j|i}+p_{j|i}}{2N}
\end{eqnarray*}
The union of $k$-th order neighbor set are found in $O(min(|V|,(|E|/|V|)^k)|V|)$ using Breadth-First-Search.
Our method use the nearest neighbor set to approximate topological similarity in $O(K|V|)$ time.

\subsection{Layout Proximity}
For layout proximity, we measure the probability of the pair $(y_i,y_j)$ in the layout space with Student's t-distribution and Euclidean distance.
The Student's t-distribution is employed by t-SNE to capture local proximity within groups.
Therefore, layout proximity can be reformulated as follows: 
$$q_{ij}=\frac{(1+ld_{ij}^2)^{-1}}{\sum_{k\not=l}(1+ld_{ij}^2)^{-1}} = \frac{(1+ld_{ij}^2)^{-1}}{Z}$$
where $Z$ denotes the normalization term.

\subsection{Distance Minimization}
In the third stage, similar vertices should be close to each other in the layout space, the optimal choice of layout is to minimize Kullback-Leibler divergences between topological similarity $P$ and layout proximity $Q$. The problem boils down to solving the following problem:
\begin{eqnarray*}
Y^* &=& \argmin_Y O(P||Q)\\
&=& \argmin_Y Dis_{KL}(P||Q)\\
&=& \argmin_Y \sum_{i\not=j} p_{ij}\log \frac{p_{ij}}{q_{ij}}\\
&=& \argmin_Y \sum_{i\not=j} p_{ij}\log p_{ij} - p_{ij}\log q_{ij}
\end{eqnarray*}
Since the first term is a constant, the problem is equivalent to the following optimization problem:
$$Y^* =  \argmin_Y O(P||Q) = \argmax_Y \sum_{i\not=j} \quad p_{ij}\log q_{ij}$$
To solve optimization problem, we randomly select two vertices and samples M negative points ($y_{j_k}$) by adopting negative sampling technique used in LargeVis. Negative sampling technique reduce distance calculation from $N$ to $M$. Therefore, the optimization problem is reformulated as follows:
\begin{eqnarray}\label{eq:objectfunction}
Y^*   &=& \argmax_Y \sum_{i\not=j} p_{ij}[\log q_{ij}+\sum\limits_{k=1}^M \gamma \log(1-q_{ij_k})]
\end{eqnarray}
The partial derivative of equation (\ref{eq:objectfunction}) by $y_j$ is derived as:
\begin{eqnarray*}
\frac{\partial O}{\partial y_i} &=& -2 F^{attr}_{ij} + \sum\limits_{k=1}^M \gamma F^{rep}_{ij_k}\\
F^{attr}_{ij} &=& \frac{p_{ij}ld_{ij}}{1+ld_{ij}^2}\\
F^{rep}_{ij_k} &=& \frac{\gamma (y_i-y_{j_k})}{ld_{ij_k}^2(1+ld_{ij_k}^2)}
\end{eqnarray*}

The gradient shows that each vertex receives $1$ attractive force and $M$ repulsive forces. In this way, graph layout methods by LargeVis is a special case of spring-electrical model.
